BayesWipe: A Scalable Probabilistic Framework for Cleaning BigData

Recent efforts in data cleaning of structured data have focused exclusively on problems like data deduplication, record matching, and data standardization; none of the approaches addressing these problems focus on fixing incorrect attribute values in tuples. Correcting values in tuples is typically performed by a minimum cost repair of tuples that violate static constraints like CFDs (which have to be provided by domain experts, or learned from a clean sample of the database). In this paper, we provide a method for correcting individual attribute values in a structured database using a Bayesian generative model and a statistical error model learned from the noisy database directly. We thus avoid the necessity for a domain expert or clean master data. We also show how to efficiently perform consistent query answering using this model over a dirty database, in case write permissions to the database are unavailable. We evaluate our methods over both synthetic and real data.

==> bw_ack.tex <==
%!TEX root = bw_journal.tex
%\vspace{-0.1in}
\section*{Acknowledgments}
We thank Dr. K. Sel\c cuk Candan for his valuable advice, and Preet Inder Singh Rihan for his help with probabilistic databases. This research is supported in part
by the ONR grants N00014-13-1-0176, N0014-13-1-0519, ARO grant W911NF-13-1-0023 and a Google Research
Grant.
\vspace{-0.14in}

